Future-Proofing Mobile Networks: A Digital Twin Approach to Multi-Signal Management

Digital Twins (DTs) are set to become a key enabling technology in future wireless networks, with their use in network management increasing significantly. We developed a DT framework that leverages the heterogeneity of network access technologies as a resource for enhanced network performance and management, enabling smart data handling in the physical network. Tested in a Campus Area Network environment, our framework integrates diverse data sources to provide real-time, holistic insights into network performance and environmental sensing. We also envision that traditional analytics will evolve to rely on emerging AI models, such as Generative AI (GenAI), while leveraging current analytics capabilities. This capacity can simplify analytics processes through advanced ML models, enabling descriptive, diagnostic, predictive, and prescriptive analytics in a unified fashion. Finally, we present specific research opportunities concerning interoperability aspects and envision aligning advancements in DT technology with evolved AI integration.

==> challenges.tex <==
%BACK UP OF GEN AI CHALLENGES PART
\textbf{The Role of GenAI: Language Models.} GenAI, particularly advanced language models (LMs), can present significant opportunities for enhancing interoperability, integration, and expansion of DTs. One of the critical capabilities of these models is their proficiency in generating code, which can be harnessed to facilitate seamless interaction between different DT components. For example, when integrating a new DT capability provided by another supplier, LMs can automatically generate the necessary interfacing code (e.g., API), ensuring that various components can communicate and work together effectively. Moreover, these models have demonstrated the potential to operate on smaller devices, such as smartphones and IoT devices \cite{jung2024optimizing}. This opens up possibilities for these models to assist in real-time when a device needs to be accommodated into a new DTs. For instance, the LM can dynamically generate and execute the code required to integrate the device into the existing DT architecture, ensuring consistent integration into the DTs. Similarly, devices belonging to the physical network can fine-tune their locally stored code applications, which can include sensing capabilities, analytics, or other functionalities, by deriving insights from the DT itself. However, it is worth noting that LMs are not infallible. Their broad knowledge and general capabilities sometimes result in outputs that are not perfectly suited for specific cases, leading to potential errors and inaccuracies, including for the case of code generation. It is essential to anticipate these limitations and develop robust recovery mechanisms to manage and rectify inaccuracies effectively when integrating LMs into DTs. To address potential inefficiencies, inaccuracies, inconsistencies, and faults, it is crucial to implement mechanisms that allow for automated testing in controlled environments, rollback processes to revert to stable states, and feedback loops for continuous improvement \cite{tarkoma2023ai}. This applies especially to more constrained devices, where LMs are less knowledgeable than cloud-based LMs.
\\
\\
\textbf{The Role of GenAI: Multi-modal Models.} New emerging AI models, which integrate and process multiple types of data inputs such as text, images, audio, and sensor data, might offer another layer of innovation of DTs. 
%These models can be employed to develop advanced multi-agent systems that facilitate robust interaction between the physical network and its digital twin counterpart. By leveraging the diverse data inputs, multi-modal models can provide a comprehensive and holistic understanding of the network environment. For example, combining sensor data with network telemetry and environmental context allows for more accurate and refined analytics, possibly leading to better decision-making and optimization. In a practical scenario within UbiKampus, consider a situation where the DT integrates data from motion detectors, air quality sensors, Wi-Fi access points, thermal cameras, and network telemetry. By analyzing this combined data, the DT can identify, at once, patterns of workspace utilization, detect areas with poor air quality, monitor network congestion, and even assess temperature distributions within the space. For instance, if the motion detectors, Wi-Fi access points, and thermal cameras indicate that a particular meeting room is frequently occupied but the air quality sensors report high levels of CO2 and the thermal cameras detect elevated temperatures, the DT can trigger actions to improve ventilation and adjust the room’s climate control systems. Simultaneously, network telemetry data might reveal that the Wi-Fi network is experiencing high traffic during these meetings. The DT could then optimize network resource allocation to ensure a stable and efficient connection for all users. The significant advancement with multi-modal models is that previously, achieving such comprehensive analysis would have required multiple AI models and additional models or human intervention to find correlation patterns. Now, this can be done in a unified fashion through the use of a multi-modal model, which can process and integrate diverse data types seamlessly, providing a more efficient and cohesive solution for managing and optimizing the network environment. 
These models can be employed to develop advanced multi-agent systems that facilitate robust interaction between the physical network and its DT counterpart. By leveraging the diverse data inputs, multi-modal models can provide a comprehensive and holistic understanding of the network environment, which otherwise would require multiple AI models and additional models or human intervention to find correlation patterns. Now, this can be done in a unified fashion through the use of a multi-modal model, which can process and integrate diverse data types seamlessly, providing a more efficient and cohesive solution for managing and optimizing the network environment.
However, a significant challenge in leveraging multi-modal models is ensuring that the data provided are meaningful and consistent in this multi-modal setting. It is essential that the DTs, and even the physical network part, can understand and validate the relevance and accuracy of the multi-modal data to avoid inconsistencies in interpreting the surrounding context. Additionally, multi-modal models tend to be more expensive in terms of operational expenditure (OPEX) because they rely on more complex models and larger datasets. The increased complexity and resource requirements must be carefully managed to balance performance and cost-effectiveness. Furthermore, with the current state of the art, it is not feasible to expect real-time operations from multi-modal models due to their slower inference processing. This limitation restricts their application in scenarios requiring immediate response and control, emphasizing the need for ongoing research and development to improve the speed and efficiency of these models.

==> old_DT_framework_in_Action.tex <==
\section{The DT Framework in Action}

Figure \ref{fig:dtgraph} demonstrates the practical application of our DT framework within UbiKampus. The bottom-left part of the figure illustrates the network configuration sensed by a single smartphone device, which includes multiple networks such as LTE, Wi-Fi, and Bluetooth (the illustration is a snapshot taken from what is shown in the Network Twin Console). This setup highlights how the proposed framework captures the diverse network signals a device can detect.

The bottom-right part of the figure showcases the signal information gathered by an application running on a mobile device. In this particular scenario, as we include smartphones as end-devices, we developed it as an Android application. However, given the portability of the data modeling and API of our framework, this can be easily adapted to other types of devices.%, including very constrained IoT devices, assuming that these have the capability of relying on device management protocols, such as LwM2M, and standardized data models.
The application continuously receives and streams incoming signals from the end-device. Built on top of the open-source project netmonster-core\footnote{\url{https://github.com/mroczis/netmonster-core}}, the application periodically sends the data via MQTT to the Signal Handler, which pre-processes the data and publishes it via the DT platform to the Network Twin Console, which displays the received signal information.

Considering this particular example shown at the bottom of Figure \ref{fig:dtgraph}, the application running on End-Devices provides detailed real-time metrics, such as network type, frequency, and signal strength, and various network parameters like RSSI and RSRP, which are essential for the DT's operational analytics (and in turn of the network management). While this example specifically shows the case of mobile network connectivity KPIs, the system is capable of transferring and, in turn, representing in the DT system key KPIs from other RATs in the form shown in Figure \ref{fig:signals}. %In the bottom part of the figure, it is possible to observe those metrics reflected also in our DT visualization system.

%This comprehensive signal handling allows the DT to have a full overview of the network capabilities of the physical network, enabling more comprehensive and intelligent analytics. %By providing a holistic view of the network environment, the DT framework can then perform sophisticated analysis and optimization, enhancing overall network performance and management.

==> table.tex <==

\begin{table*}[]
\begin{tabularx}{\textwidth}{X|X|X}
\cline{2-3}
\textbf{} & \textbf{Challenges \& Opportunities} & \textbf{Explanation} \\ \hline

% First row
\textbf{Inter- and Intra-Interoperability} & \textbf{Opportunity:} DT interoperability & DTs-interoperability can enhance global feature learning, allowing for aggregation and analysis of data from diverse sources to improve the accuracy and effectiveness of the DT models and their respective physical counterparts. Moreover, the ability to easily incorporate new end-devices and types of connectivity through \textit{plug-and-play} functionality is a significant opportunity. \\ \hline

% Third row
\textbf{Standardized Data Models for Enhanced Interoperability} & \textbf{Opportunity:} Data interoperability & By adopting a strategy similar to OneDM\footnote{\url{https://onedm.org/}}, which aims to establish common data and interaction models for IoT devices, we can seek to create a unified data model for DTs. Such a model would enable various systems to work together without the need for complex data conversion processes. This standardization would facilitate easier and more reliable integration of diverse data sources, enhancing the overall functionality and performance of DT architectures.  \\ \hline


% Third row
\multirow{3}{*}{\textbf{\makecell{The Role of GenAI:\\Language Models}}} & \textbf{Opportunity:} Facilitating seamless interaction between different DT components & Integrating a new DT capability provided by another supplier, LMs can automatically generate the necessary interfacing code (e.g., API), ensuring that various components can communicate and work together effectively. \\

\cline{2-3} & \textbf{Opportunity:} Code fine-tuning & Devices belonging to the physical network can fine-tune their locally stored code applications via LMs, which can include sensing capabilities, analytics, or other functionalities, by deriving insights from the DT itself.  \\ 

\cline{2-3} & \textbf{Challenge:}  Hallucinations & LM broad knowledge and general capabilities sometimes result in outputs that are not perfectly suited for specific cases, leading to potential errors and inaccuracies, including for the case of code generation. Therefore, it is essential to anticipate these limitations and develop robust recovery mechanisms to manage and rectify inaccuracies effectively when integrating LMs into DTs. \\ 


\hline
\end{tabularx}
\end{table*}

\begin{table*}[]
\begin{tabularx}{\textwidth}{X|X|X}
\cline{2-3}
\textbf{} & \textbf{Challenges \& Opportunities} & \textbf{Explanation} \\ \hline
% Fourth row
\multirow{4}{*}{\textbf{\makecell{The Role of GenAI: \\ Multi-modal Models}}} & \textbf{Opportunity:} Provisioning a comprehensive and holistic understanding of the environment & Combining sensor data with network telemetry and environmental context allows for more accurate and refined analytics, possibly leading to better decision-making and optimization. \\

\cline{2-3} & \textbf{Opportunity:} Reduced number of needed AI models & Previously, achieving such comprehensive analysis would have required multiple AI models and additional models or human intervention to find correlation patterns. Now, this can be done in a unified fashion through the use of a multi-modal model, which can process and integrate diverse data types seamlessly, providing a more efficient and cohesive solution for managing and optimizing the network environment. \\ 

\cline{2-3} & \textbf{Challenge:} Data consistency & It is essential that the DTs, and even the physical network part, can understand and validate the relevance and accuracy of the multi-modal data to avoid inconsistencies in interpreting the surrounding context. \\

\cline{2-3} & \textbf{Challenge:} Operational expenditure (OPEX) & The increased complexity and resource requirements must be carefully managed to balance performance and cost-effectiveness. Furthermore, with the current state of the art, it is not feasible to expect real-time operations from multi-modal models due to their slower inference processing. This limitation restricts their application in scenarios requiring immediate response and control, emphasizing the need for ongoing research and development to improve the speed and efficiency of these models. \\

\hline           

\end{tabularx}
\end{table*}
